Operational Characterization of a Public Scientific Datacenter During and Beyond the COVID-19 Period

Datacenters are imperative for the digital society. They offer services such as computing, telecommunication, media, and entertainment. Datacenters, however, consume a lot of power. Thus, Improving datacenter operations is important and may result in better services, reduced energy consumption and reduced costs. To improve datacenters, we must understand what is going on inside them. Therefore, we use operational traces from a scientific cluster in the Netherlands to investigate and understand how that cluster operates. Due to work-from-home circumstance, the covid period might have changed our daily usage of online applications, such as zoom and google meet. In this research, we focus on the operations of a scientific cluster (LISA) inside the SURF datacenter. The global pandemic might have changed how the LISA cluster operates. To understand the change, we collect, combine, and analyze operational logs from the LISA cluster. The tool to collect the data that belongs to the non-covid period was accomplished in previous research. Nonetheless, both the tool and instrument to combine and analyze the traces are lacking. This research focuses on designing an instrument that can combine and analyze the traces during and before the coronavirus period. The instrument can also produce graphs for customarily selected rack, nodes and periods. Moreover, we characterize the traces that belong to the coronavirus period using the scientific instrument and additional tools. The outcome of this research helps us understand how the operations for a scientific cluster (LISA) in the Netherlands has changed after the global pandemic.

==> project_card.tex <==
\section*{The Project Card}
% \begin{enumerate}
%     \item Research question(s)
%     \item Approach, emphasis on methods
%     \item Main results and contribution(s)
% \end{enumerate}

\begin{framed}

Research question(s):
\begin{description}
    \item[RQ1] How to design an instrument that can statistically compare the workload of a datacenter across different time periods? \\
    
    \item[RQ2] Are there significant differences between the datacenter operations before and during coronavirus periods? \\
  
    \item[RQ3] How can we characterize in detail (low-level) workloads and operations  during the coronavirus period. \\
\end{description}
\end{framed}

\begin{framed}
Research method(s):
\begin{description}
    \item[M1] Design and develop and instrument that can produce results using basic statistical methods for two different time periods.\\
    \item[M2] Develop additional scripts that depicts the general utilization levels for the covid and non-covid periods.
\end{description}

Research approach:
\begin{description}
    \item[A1] To address {\bf RQ3}, we use the scientific instrument and additional scripts to produce curves and violin plots for the covid and non-covid period. \\
    
    \item[A2] To address {\bf RQ2}, we interpret the covid period of the graphs and compare them to the non-covid period. \\
    
    \item[A3] To address {\bf RQ1} we use methodology M1 and develop an instrument that can statistically compare the operations of a cluster across different time periods.
\end{description}
    
\end{framed}

\newpage
Main results and contribution:
\begin{framed}
\begin{description}

    \item[R1] A presentation of the material, probably presented at the @Large research team \\
    \item[R2] Finding out how the operations of LISA has changed for certain metrics during the covid period. \\
    
    \item[C1] An instrument that can compare the covid and non-covid period using basic statistical methods. \\
    \item[C2] An instrument that can produce results for customarily select nodes, rack, or time period. \\
    
\end{description}
\end{framed}

